Hypothesis Testing for Hierarchical Structures in Cognitive Diagnosis Models

Cognitive Diagnosis Models (CDMs) are a special family of discrete latent variable models widely used in educational, psychological and social sciences. In many applications of CDMs, certain hierarchical structures among the latent attributes are assumed by researchers to characterize their dependence structure. Specifically, a directed acyclic graph is used to specify hierarchical constraints on the allowable configurations of the discrete latent attributes. In this paper, we consider the important yet unaddressed problem of testing the existence of latent hierarchical structures in CDMs. We first introduce the concept of testability of hierarchical structures in CDMs and present sufficient conditions. Then we study the asymptotic behaviors of the likelihood ratio test (LRT) statistic, which is widely used for testing nested models. Due to the irregularity of the problem, the asymptotic distribution of LRT becomes nonstandard and tends to provide unsatisfactory finite sample performance under practical conditions. We provide statistical insights on such failures, and propose to use parametric bootstrap to perform the testing. We also demonstrate the effectiveness and superiority of parametric bootstrap for testing the latent hierarchies over non-parametric bootstrap and the na\"ive Chi-squared test through comprehensive simulations and an educational assessment dataset.

==> testing_hierarchy.wordcount.tex <==
File: testing_hierarchy.tex
Encoding: utf8
Sum count: 10034
Words in text: 8933
Words in headers: 55
Words outside text (captions, etc.): 344
Number of headers: 14
Number of floats/tables/figures: 21
Number of math inlines: 658
Number of math displayed: 44
Subcounts:
  text+headers+captions (#headers/#floats/#inlines/#displayed)
  202+10+0 (2/0/0/0) _top_
  1021+1+0 (1/0/1/0) Section: Introduction\}\textbackslash{}label\{chap1-sec-intro
  62+4+0 (1/0/13/0) Section: Model Setup and Motivations
  775+3+3 (1/1/68/3) Subsection: Cognitive Diagnosis Models\}\textbackslash{}label\{chap1-sec-CDM
  400+3+38 (1/3/31/1) Subsection: Problem and Motivations
  2279+4+5 (1/1/280/13) Section: Testability Requirements and Conditions
  203+3+0 (1/0/2/0) Section: Likelihood Ratio Test
  1497+6+75 (1/1/127/16) Subsection: Failure of Limiting Distribution of LRT
  432+8+0 (1/0/77/11) Subsection: Likelihood Ratio Test for General Latent Class Models 
  1173+4+169 (1/9/21/0) Subsection: Bootstrap and Numerical Studies
  624+3+26 (1/2/37/0) Section: Real Data Analysis
  265+1+0 (1/0/1/0) Section: Discussions
  0+5+28 (1/4/0/0) Section: Supplementary Material: Additional Simulation Results


